High-resolution Bayesian mapping of landslide hazard with unobserved trigger event

Statistical models for landslide hazard enable mapping of risk factors and landslide occurrence intensity by using geomorphological covariates available at high spatial resolution. However, the spatial distribution of the triggering event (e.g., precipitation or earthquakes) is often not directly observed. In this paper, we develop Bayesian spatial hierarchical models for point patterns of landslide occurrences using different types of log-Gaussian Cox processes. Starting from a competitive baseline model that captures the unobserved precipitation trigger through a spatial random effect at slope unit resolution, we explore novel complex model structures that take clusters of events arising at small spatial scales into account, as well as nonlinear or spatially-varying covariate effects. For a 2009 event of around 4000 precipitation-triggered landslides in Sicily, Italy, we show how to fit our proposed models efficiently using the integrated nested Laplace approximation (INLA), and rigorously compare the performance of our models both from a statistical and applied perspective. In this context, we argue that model comparison should not be based on a single criterion, and that different models of various complexity may provide insights into complementary aspects of the same applied problem. In our application, our models are found to have mostly the same spatial predictive performance, implying that key to successful prediction is the inclusion of a slope-unit resolved random effect capturing the precipitation trigger. Interestingly, a parsimonious formulation of space-varying slope effects reflects a physical interpretation of the precipitation trigger: in subareas with weak trigger, the slope steepness is shown to be mostly irrelevant.

==> mylatex.tex <==
%latex shortcuts
%Thomas Opitz
%(taken over from Anthony Davison's "macros.tex" file)

%simple shortcuts
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}

\def\rm#1{\mathrm{#1}}
\def\rmd{\mathrm{d}}

\def\vhalf{\vspace{\stretch{0.5}}}
\def\vone{\vspace{\stretch{1}}}
\def\vtwo{\vspace{\stretch{2}}}
\def\vthree{\vspace{\stretch{3}}}

\def\pr{\mathrm{pr}}

\def\calA{{\mathcal A}}
\def\calB{{\mathcal B}}
\def\calC{{\mathcal C}}
\def\calD{{\mathcal D}}
\def\calE{{\mathcal E}}
\def\calF{{\mathcal F}}
\def\calG{{\mathcal G}}
\def\calH{{\mathcal H}}
\def\calI{{\mathcal I}}


\def\auml{{\"a}}
\def\euml{{\"e}}
\def\uuml{{\"u}}


%redefine commands
\def\bar#1{\overline{#1}}

% \def\half{{\textstyle{1\over 2}}}
% \def\third{{\textstyle{1\over 3}}}
% \def\quarter{{\textstyle{1\over 4}}}
% \def\sixth{{\textstyle{1\over 6}}}
% \def\frac#1#2{{\textstyle{#1\over#2}}}
% \def\Beta{{\rm B}}

% \def\argmin{{\rm argmin}}  
% \def\diag{{\rm diag}}  
% \def\mod{{\rm mod}}  
% \def\tr{{\rm tr}}
% \def\sign{{\rm sign}}
% \def\ow{{\rm otherwise}}  
% \def\obs{{\rm obs}}  
% \def\endex{{\hfill{\color{red}$\bullet$}\medskip}}
% \def\Endex{{\hfill{$\bullet$}\medskip}}
% \def\redbf#1{{\color{red}\bf #1}}%
% \def\red#1{{\color{red} #1}}%
% \def\white#1{{\color{black} #1}}%

% \DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
% \DeclareMathSymbol{\Natural}{\mathbin}{AMSb}{"4E}
% \DeclareMathSymbol{\Integer}{\mathbin}{AMSb}{"5A}
% \DeclareMathSymbol{\Real}{\mathbin}{AMSb}{"52}
% \DeclareMathSymbol{\Rational}{\mathbin}{AMSb}{"51}
% \DeclareMathSymbol{\Imaginary}{\mathbin}{AMSb}{"49}
% \DeclareMathSymbol{\Complex}{\mathbin}{AMSb}{"43} 
% \DeclareMathSymbol{\Disk}{\mathbin}{AMSb}{"44} 
% \def\bi{\begin{itemize}}
% \def\ei{\end{itemize}}
% \def\bd{\begin{description}}
% \def\ed{\end{description}}
% \def\ben{\begin{enumerate}}
% \def\een{\end{enumerate}}
% \def\bv{\begin{verbatim}}
% \def\ev{\end{verbatim}}

% \def\bth{{$b{\rm th}$ }}
% \def\cth{{$c{\rm th}$ }}
% \def\dth{{$d{\rm th}$ }}
% \def\fth{{$f{\rm th}$ }}
% \def\gth{{$g{\rm th}$ }}
% \def\hth{{$h{\rm th}$ }}
% \def\ith{{$i{\rm th}$ }}
% \def\jth{{$j{\rm th}$ }}
% \def\kth{{$k{\rm th}$ }}
% \def\lth{{$l{\rm th}$ }}
% \def\mth{{$m{\rm th}$ }}
% \def\nth{{$n{\rm th}$ }}
% \def\pth{{$p{\rm th}$ }}
% \def\rth{{$r{\rm th}$ }}
% \def\sth{{$s{\rm th}$ }}
% \def\tth{{$t{\rm th}$ }}
% \def\uth{{$u{\rm th}$ }}
% \def\vth{{$v{\rm th}$ }}
% \def\wth{{$w{\rm th}$ }}

% \def\calA{{\mathcal A}}
% \def\calL{{\mathcal L}}
% \def\calB{{\mathcal B}}
% \def\calC{{\mathcal C}}
% \def\calD{{\mathcal D}}
% \def\calE{{\mathcal E}}
% \def\F{{\mathcal F}}
% \def\G{{\mathcal G}}
% \def\H{{\mathcal H}}
% \def\calH{{\mathcal H}}
% \def\IG{{\mathcal IG}}
% \def\cI{{\mathcal I}}
% \def\cP{{\mathcal P}}
% \def\calJ{{\mathcal J}}
% \def\calK{{\mathcal K}}
% \def\calM{{\mathcal M}}
% \def\calN{{\mathcal N}}
% \def\N{{\calN}}
% \def\calP{{\mathcal{P}}}
% \def\calO{{\mathcal{O}}}
% \def\calS{{\mathcal{S}}}
% \def\calI{{\mathcal{I}}}
% \def\calR{{\mathcal R}}
% \def\calT{{\mathcal T}}
% \def\calU{{\mathcal U}}
% \def\calV{{\mathcal V}}
% \def\calW{{\mathcal W}}
% \def\calX{{\mathcal X}}
% \def\calY{{\mathcal Y}}
% \def\calZ{{\mathcal Z}}
% \def\W{{\mathcal W}}
% \def\U{{\Upsilon}}
% \def\f{\frac}
% \def\l{{\lambda}}
% \def\d{{\delta}}
% \def\bX{{\bar X}}
% \def\s{{\sigma}}
% \def\p{{\partial}}
% \def\p{{d}}
% \def\v{{\varepsilon}}
% \def\dis{{\displaystyle}}
% \def\a{{\alpha}}
% \def\b{{\beta}}
% \def\hash{{\#}}
% \def\bar#1{{\overline{#1}}}
% \def\hat#1{{\widehat{#1}}}
% \def\barY{{\overline{Y}}}
% \def\barX{{\overline{X}}}
% \def\barZ{{\overline{Z}}}
% \def\barx{{\overline{x}}}
% \def\bary{{\overline{y}}}
% \def\barz{{\overline{z}}}
% \def\T{{ \mathrm{\scriptscriptstyle T} }}
% \def\mT{{ -\mathrm{\scriptscriptstyle T} }}
% \newcommand{\indep}{\perp\!\!\!\perp}
% \newcommand{\nindep}{\perp\!\!\!\perp\!\!\!\!\!\!/\;\;}

% \newcommand{\med}{{\rm med}}
% \newcommand{\card}{{\rm card}}
% % \newcommand{\do}{{\rm do}}
% \newcommand{\Splus}{\textsc{S-Plus}\ }
% %\newcommand{\R}{\texttt{R} }

% % statistical notation

% \def\rmi{{\rm i}}
% \def\pr{{\rm Pr}}
% \def\Pr{\pr}
% \def\E{{\rm E}}
% \def\Ev{{\rm Ev}}
% \def\var{{\rm var}}
% \def\cov{{\rm cov}}  
% \def\corr{{\rm corr}}  
% \def\Estar{{\rm E^*\thinspace}}
% \def\varstar{{\rm var^*\thinspace}}
% \def\covstar{{\rm cov^*\thinspace}}  
% \def\median{{\rm median}}  
% \def\cum{{\rm cum}}
% \def\IMSE{{\rm IMSE}}  
% \def\AIC{{\rm AIC}}  
% \def\BIC{{\rm BIC}}  
% \def\NIC{{\rm NIC}}  
% \def\AICc{{\rm AIC_c}}  
% \def\CV{{\rm CV}}  
% \def\GCV{{\rm GCV}}  
% \def\IQR{{\rm IQR}}  
% \def\MAD{{\rm MAD}}  
% \def\Lik{{L}}
% \def\logL{{\ell}}
% \def\RLik{{RL}}
% \def\logLp{{\ell_{\rm p}}}

% \def\Dto{{\ {\buildrel D\over \longrightarrow}\ }}
% \def\Pto{{\ {\buildrel P\over \longrightarrow}\ }}
% \def\rto{{\ {\buildrel r\over \longrightarrow}\ }}
% \def\2to{{\ {\buildrel 2\over \longrightarrow}\ }}
% \def\Wto{{\ {\buildrel W\over \longrightarrow}\ }}
% \def\psto{{\ {\buildrel \rm{p.s.}\over \longrightarrow}\ }}
% \def\asto{{\ {\buildrel \rm{a.s.}\over \longrightarrow}\ }}
% \def\iid{{\ {\buildrel \rm{iid}\over \sim}\ }}
% \def\ind{{\ {\buildrel \rm{ind}\over \sim}\ }}
% \def\dotsim{{\ {\buildrel \cdot\over \sim}\ }}
% %\def\sim{{\ {\sim}\ }}
% %\def\to{{\longrightarrow}}
% \def\Deq{{\ {\buildrel D\over =}\ }}
% \def\Eoneton{{$E_1,\ldots,E_n$}}
% %\def\T1ton{{$T_1,\ldots,T_n$}}
% \def\I1ton{{$I_1,\ldots,I_n$}}
% %\def\U1ton{{$U_1,\ldots,U_n$}}
% \def\X1ton{{$X_1,\ldots,X_n$}}
% \def\Y1ton{{$Y_1,\ldots,Y_n$}}
% \def\Z1ton{{$Z_1,\ldots,Z_n$}}
% \def\R1ton{{$R_1,\ldots,R_n$}}
% \def\e1ton{{$e_1,\ldots,e_n$}}
% \def\t1ton{{$t_1,\ldots,t_n$}}
% \def\x1ton{{$x_1,\ldots,x_n$}}
% \def\y1ton{{$y_1,\ldots,y_n$}}
% \def\z1ton{{$z_1,\ldots,z_n$}}
% %\def\r1ton{{$r_1,\ldots,r_n$}}

% % Journal abbreviations

% \def\AAP{\emph{Advances in Applied Probability}}
% \def\AnnProbab{\emph{Annals of Probability}}
% \def\AISM{\emph{Annals of the Institute of Statistical Mathematics}}
% \def\AMS{\emph{Annals of Mathematical Statistics}}
% \def\ApplStatist{\emph{Applied Statistics}}
% \def\AS{\emph{Annals of Statistics}}
% \def\B{\emph{Bernoulli}}
% \def\Bka{\emph{Biometrika}}
% \def\CJS{\emph{Canadian Journal of Statistics}}
% \def\CSDA{\emph{Computational Statistics \& Data Analysis}}
% \def\Eca{\emph{Econometrica}}
% \def\ISI{\emph{International Statistical Review}}
% \def\ISR{\emph{International Statistical Review}}
% \def\JAMA{\emph{Journal of the American Medical Association}}
% \def\JAP{\emph{Journal of Applied Probability}}
% \def\JASA{\emph{Journal of the American Statistical Association}}
% \def\JBES{\emph{Journal of Business \& Economic Statistics}}
% \def\JCGS{\emph{Journal of Computational and Graphical Statistics}}
% \def\JSCS{\emph{Journal of Statistical Computation and Simulation}}
% \def\JRSSA{\emph{Journal of the Royal Statistical Society series A}}
% \def\JRSSB{\emph{Journal of the Royal Statistical Society series B}}
% \def\JRSSD{\emph{The Statistician}}
% \def\SJS{\emph{Scandinavian Journal of Statistics}}
% \def\SPA{\emph{Stochastic Processes and their Applications}}
% \def\SM{\emph{Survey Methodology}}
% \def\SS{\emph{Statistical Science}}
% \def\TAS{\emph{The American Statistician}}
% \def\Tech{\emph{Technometrics}}
% \def\ZW{\emph{Z. Wahrsch. v. geb.}}
% \def\JC{\emph{Journal of Classification}}
% \def\PNAS{\emph{Proceedings of the National Academy of Science}}

% % utility macros

% \def\np{{\newpage}}
% \def\gap{{\vskip 0.3in}}
% \def\etal{{\sl et al.}} 
% \def\pound{{\it \$}}
% \def\apriori{{\sl a priori }}
% \def\examfoot{{\vfill\hfill{\bf Turn over}\eject}}
% \def\newtransparency{{\newpage}}
% \def\Section{{Section~}}
% \def\Sections{{Sections~}}
% \def\Pvalue{{P-value}}
% \def\Pvalues{{P-values}}

% \def\report#1{{\newpage\centerline{\bf #1}\smallskip}}

% % odds and ends

% \def\redbf#1{{\color{red}\bf #1}}%
% \def\Defn{\redbf{Definition:\ }}%
% \def\Thm#1{\redbf{Theorem #1:\ }}%
% \def\Ex#1{\redbf{Example #1:\ }}%
% \def\Note{\redbf{Note:\ }}%
% \def\Exercise#1{\redbf{Exercise #1:\ }}%
% \def\Ill{\redbf{Illustration:\ }}%
% \def\endex{{\hfill\redbf{$\bullet$}\smallskip}}
% \def\calP{{\mathcal{P}}}
% \def\calS{{\mathcal{S}}}
% \def\calI{{\mathcal{I}}}
% \def\eme{{\`eme}}
% \def\ere{{\`ere}}
% %\def\picbox#1#2{{\centerline{\psfig{figure=#1,height=#2pc}}}}%
% \def\picbox#1#2#3{{\centerline{\psfig{figure=#1,height=#2pc,angle=#3}}}}%
% \def\tt#1{{\texttt{#1}}}
% \def\Der#1{\textbf{D#1}}



==> packages.tex <==
\usepackage[english]{babel}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{bm}

